Diversification Across Mining Pools: Optimal Mining Strategies under PoW

Mining is a central operation of all proof-of-work (PoW) based cryptocurrencies. The vast majority of miners today participate in "mining pools" instead of "solo mining" in order to lower risk and achieve a more steady income. However, this rise of participation in mining pools negatively affects the decentralization levels of most cryptocurrencies. In this work, we look into mining pools from the point of view of a miner: We present an analytical model and implement a computational tool that allows miners to optimally distribute their computational power over multiple pools and PoW cryptocurrencies (i.e. build a mining portfolio), taking into account their risk aversion levels. Our tool allows miners to maximize their risk-adjusted earnings by diversifying across multiple mining pools which enhances PoW decentralization. Finally, we run an experiment in Bitcoin historical data and demonstrate that a miner diversifying over multiple pools, as instructed by our model/tool, receives a higher overall Sharpe ratio (i.e. average excess reward over its standard deviation/volatility).

==> related.tex <==


\section{Similar solutions currently available}

\panagiotis{I moved this section after the intro, however I have here parameters and notation that are referenced later}


In this section we present an overview of some of the currently available solutions that enable a miner to maximize his profit as the "reward over time" ratio $\frac{\blockreward{\cryptoid}}{\blocktime{\cryptoid}}$ and the total cryptocurrency hashrate $\totalhashrate{\cryptoid}$ fluctuate over time. Note that while these solutions have a similar goal, they do not take the miner's risk aversion $\cara$ into account.
\subsubsection{Multipoolminer}\cite{multipoolminer} is a Windows Powershell script, which performs benchmarking of CPUs or GPUs in the system while continusly monitors a pre-defined set of mining pools that support multiple PoW mining algorithms (e.g. Miningpoolhub). By executing the script, the miner can maximize his profit based on the "reward over time" ratio $\frac{\blockreward{\cryptoid}}{\blocktime{\cryptoid}}$ (which is mostly determined by each cryptocurrency $\cryptoid$ exchange rate), the total cryptocurrency hashrate $\totalhashrate{\cryptoid}$ and the miner's benchmarked total mining power for each PoW algorithm $\minertotalalgrate{\powalg{i}}$. While Multipoolminer does not take a risk aversion factor into account, it supports mining on a secondary PoW algorithm simultaneously (known as ``dual-mining"), in a similar way we describe in section \ref{multi-crypto-multi-pow}. \foteini{Between different cryptocurrencies? Explain in text what dual mining is (no reference required)} \panagiotis{Done.} Then the miner can have his earnings converted to a single chosen cryptocurrency automatically by the pool. Multipoolminer, being a Windows Powershell script, is not compatible with ASIC miners which are commonly based on embedded Linux systems.
\foteini{Miner portfolio within the Multipool pool. Can you write the Bitcoin percentage? } \panagiotis{It seems that Multipoolminer no longer supports Multipool pool, it supports other pools though that have multiple pow cryptos, so I reworded and generalized the whole paragraph.}

\subsubsection{Minergate}\cite{minergate} is a multi-cryptocurrency mining pool that also offers its own GUI miner tool. The tool offers a "smart mining" functionality, which in a similar fashion with Multipoolminer, automatically selects the most "profitable" cryprocurrency to mine. To accomplish this, it also performs a benchmarking of CPUs or GPUs in the system to calculate the total mining power for each PoW algorithm $\minertotalalgrate{\powalg{i}}$. The pool also offers the choice between PPS and PPLNS reward systems for each cryptocurrency, however it doesn't take the exchange rate fluctuations into account, requiring manual user intervention.
\foteini{is it same idea as before? dual mining?} \panagiotis{Yes same idea as multipoolminer,only difference it's an "all-in-one" tool (miner+pool+wallet)}


\subsubsection{Smartmine}\cite{smartmine} offers a GUI tool that works similar with Multipoolmine, however it offers an additional functionality of automatically converting coins into USD and paying the user into a Paypal or Amazon wallet.
\\ \\
Other notable solutions include Nicehash, WinMiner, and Awesome Miner, all of which aim to maximize the miner's profit by selecting the most profitable cryptocurrency based on the some or all of the above parameters. However, to our knowledge, no other solution exists that offers the miner's risk aversion $\cara$ as an input parameter.

\section{Related work}
In this section we provide an overview of the literature related to mining pools as follows:
\subsection{Optimal mining pool operation}
B. Fisch, R. Pass and a. shelat\cite{10.1007/978-3-319-71924-5_15} examined the problem of a pool allocating block rewards to its participants to maximize their "social welfare", defined to be the pool's steady-state utility. Complementary to \cite{jiasun}, it provides a top-down (from the pool's point of view) analysis, where the optimization problem becomes maximizing the pool's shares utility, under a fixed block reward. According to this work, the geometric pay method (which is a generalized PPS pay method, based on the same idea of Slush's pool "score" system) achieves the optimal "social welfare", under the assumption that the pool miners are risk averse, an assumption that is used in \cite{jiasun} and in our work.
\\
Y.Lewenberg et.al \cite{Lewenberg:2015:BMP:2772879.2773270} examined pooled mining mainly from a network performance scope (communications delay) and how the network delay incentivizes miners switching among pools to optimize their payoffs, due to the non-linearity introduced. This work predicts the use of autonomous agents (software) that would implement automated pool switching as the network parameters change due to growth in the Bitcoin network.
\foteini{from the point of view of the miner}
X.Liu et.al \cite{8326513} discussed the dynamic mining pool selection problem in a blockchain network, related to the computation power (hash rate) and the network's propagation delay. It assumes the choosing of a block mining strategy from the pools as in \cite{10.1007/978-3-319-71924-5_15} and provides an analysis for a two-pool blockchain network. \foteini{is this on miners side? why related to pass et al?} \panagiotis{Miners' side yes. It has the assumption that "each mining pool may adopt a different arbitrary block mining strategy" which refers to pass et al} \foteini{so no risk aversion here?}

\subsection{Analysis of reward systems}
M.Rosenfeld \cite{DBLP:journals/corr/abs-1112-4980} provided an extended technical analysis on pool mining reward systems like proportional, PPS, geometric and score-based. In addition, it includes analysis for some of advanced variants of those systems, as well as for non-standard or hybrid systems. This also discusses possible attack vectors (e.g pool-hopping and block-withholding attacks), and how mining pools can defend from such attacks. 
\\
O.Schrijvers et.al \cite{FC:SBBR16} examined the incentive compatibility of existing pool reward systems. It showed how the proportional reward system is not incentive compatible, while the PPS and PPLNS systems are incentive compatible (i.e. if and how a miner would benefit from delaying to report his shares). This work also proposed a new incentive compatible reward scheme, which satisfies proportional payments.

\subsection{Mining attacks}
Y.Zolotavkin, J.Garcia and C.Rudolph \cite{10.1007/978-3-319-68711-7_2} proposed a game theoretical model of delays in PPLNS pool reward systems, where miners can dishonestly increase their earnings by delaying the share reports in the pool closer to the end of the mining round. It then discusses how the PPLNS scheme can be incentive compatible, when there is a Nash equilibrium among the miners that will not delay reporting of their shares to the pool.
\\
I.Eyal and E.Sirer \cite{FC:EyaSir14}  presented the Seflish-mining attack, where a group of colluding miners controlling more than 1/4 but less than 1/2 of the network power could increase their earnings by strategically publishing mined blocks, while A.Sapirshtein, Y.Sompolinsky and A.Zohar \cite{FC:SapSomZoh16} further analyzed the threshold to launch a profitable selfish-mining attack.
\\
I.Eyal \cite{SP:Eyal15} discussed pool infiltration-sabotage attacks (seemingly joining pools without sharing proofs of work) and block-withholding attacks. This work's analysis showed that while these self-destructing attacks are not in the common interest of the whole cryptocurrency ecosystem, the fact that no observed attacks have been observed does not imply a Nash equilibrium, as the "anonymous" nature of the attack results in an unstable situation.
\\
Y.Sompolinsky and A.Zohar \cite{Sompolinsky:2017:BUI:3155112.3168362} provided a historical overview of cryptocurrency economics and the underlying reasons that led to the formation of mining pools, while also discussing attacks such as "pool-hopping" and "block-withholding", the centralization introduced by the pools and possible disincentives to dissolve pools.

\subsection{Improving pool operation}
\foteini{protocols to improve interaction between pools and their miners}
The stratum bitcoin mining protocol\cite{slushpool}, used in other cryptocurrencies as well, was implemented to provide low-latency communication between pool operators and members. Higher performance ASICS could then overcome the bottleneck problem of idling on network latencies, a problem which was not experienced with lower-rate CPU or GPU mining. The protocol can theoretically serve 18 Exa-hashes/s from a single TCP connection.\\
P2pool \cite{p2pool} is a decentralized Bitcoin mining pool, based on the same peer-to-peer model as Bitcoin. It creates a peer-to-peer network of miner nodes which work on a chain of shares, in a similar fashion to a blockchain, where each node works on a block that includes payouts to the previous shares' owners and the node itself. Because of its decentralized nature, there is no central point of failure, making it DoS resistant, and also it removes the central point of trust, helping against 51\% attacks, although the protocol is more resource and bandwidth intensive compared to "classic" pool mining.
\subsection{Other}
D.Huang, K.Levchenko and A.Snoeren \cite{Huang2018EstimatingPO} used historical data to estimate an investor's potential profitability by investing into cryptocurrency mining \foteini{do they consider solo mining or pools?} \panagiotis{They don't seem to specify, pooled mining is implied from sect 3} versus buying cryptocurrency coins, and the variance of each potential profitability across multiple crytocurrencies. These blockchain data, combined with daily trade statistics, were used to generate simulations of mining or speculating among 18 different ``lesser" cryptocurrencies, compared the results agains ``major" cryptocurrencies (Bitcoin and Litecoin) and retroactively determine the miner's best strategy.\foteini{how does this compares to us?} \panagiotis{Similarities: 1. We both used historical blockchain data to retroactively extract results (although they also used "trade data") Differences: 1. Their main focus is to compare mining vs buying coins 2. They don't use pools 3. They don't have a metric for risk aversion, they just use standard deviation as a risk metric 4. They used data from many specific lesser cryptocurrencies}
\\
J.Bonneau et.al \cite{SP:BMCNKF15} in their Bitcoin and Cryptocurrency research survey, also included a technical overview of mining pools in their work, as well a discussion on stability and attacks on pools.
\\
B.Pontiveros, R.Norvill and R.State \cite{8406328} proposed machine learning thechniques to detect the transaction selection policy of Bitcoin mining pools from the transaction mempool. Normally a pool would select transactions offering the highest fees, in order to maximize its income, however the methodology described would detect a deviation from this standard selection policy, e.g. ignoring transactions originating from a specific country.\foteini{censoring}
\\ A.Gencer et.al \cite{DBLP:journals/corr/abs-1801-03998} studied among others the distribution of mining power in Bitcoin and Ethereum networks by collecting data from the respective blockchains, and how this distribution indicates a high degree of centralization introduced by the formation of mining pools through analysis of these data.
\\
A.Kiayias et.al \cite{Kiayias:2016:BMG:2940716.2940773} considered an "immediate-release" and a "strategic-release" game when a miner solves a block puzzle, and identified a threshold of miner's hash power for choosing a strategy. \foteini{irrespective to miners technique, i.e. pool or cryptocurrency selection}
\\
J.Kroll, I. Davey and E.Felten \cite{Kroll2013TheEO} examined the economics of mining in Bitcoin, how it can survive attacks given that all its participants behave according to their incentives, and how a dedicated attacker can "crash" the currency. They also include a discussion on how a "51\% attack" performed by a pool that accumulated such power would eventually have a limited payoff.

